An Economic Analysis of Privacy Protection and Statistical Accuracy as Social Choices

Statistical agencies face a dual mandate to publish accurate statistics while protecting respondent privacy. Increasing privacy protection requires decreased accuracy. Recognizing this as a resource allocation problem, we propose an economic solution: operate where the marginal cost of increasing privacy equals the marginal benefit. Our model of production, from computer science, assumes data are published using an efficient differentially private algorithm. Optimal choice weighs the demand for accurate statistics against the demand for privacy. Examples from U.S.\ statistical programs show how our framework can guide decision-making. Further progress requires a better understanding of willingness-to-pay for privacy and statistical accuracy.

==> app_randomized_response.tex <==
% !Tex root = ./abowd-schmutte-privacy.tex


\subsection{Randomized Response Details}
\label{app:randomized_response}
A custodian collects data from a population of individuals, $i\in\left\{1,\ldots,N\right\}$.
Each member of the population has a sensitive characteristic and an innocuous characteristic.
The sensitive characteristic is $x_{i} = Y_{i}(1)\in\left\{0,1 \right\}$, with population proportion $\PrP\left[Y_{i}(1)=1 \right] = \pi$.
This proportion, $\pi$, is the unknown population quantity of interest.
The non-sensitive characteristic is $z_{i} = Y_{i}(0)\in\left\{0,1 \right\}$ with known population proportion $\PrP\left[Y_{i}(0)=1 \right] = \mu$.
The custodian collects and publishes a mixture
\begin{equation}
	d_{i} = T_{i}Y_{i}(1) + (1-T_{i})Y_{i}(0),
	\label{eq:RR_var}
\end{equation}
where $T_{i}$ indicates whether the sensitive or the non-sensitive question was collected, with $\PrP\left[T_{i}=1 \right] = \rho$.
The responses are independent of which information is collected: $\left(Y_{i}(1),Y_{i}(0)\right)\Perp T_{i}$. We also require that the non-sensitive item be independent of the sensitive item. This is not restrictive, since the innocuous question can literally be ``flip a coin and report whether it came up heads,'' as in the original application.

The indicator $T_{i}$ is not observed. Any data analyst observes only the reported variable $d_{i}$.
However, as in a randomized controlled trial, the probability of $T_{i}$, $\rho$, is known with certainty. Furthermore, the analyst also knows the probability of the non-sensitive response, $\mu$.

Define $\widehat{\beta} = \frac{1}{N}\sum_{i}d_{i}$, the empirical mean proportion of responses of one.
Independence of $T_{i}$ implies $\E\left[\widehat{\beta}\right] = \pi\rho + \mu(1-\rho)$.
It follows that $\widehat{\pi} = \frac{\widehat{\beta}-\mu(1-\rho)}{\rho}$ is an unbiased estimator of $\pi$ with variance $\limfunc{Var}[{\widehat{\pi}}] = \limfunc{Var}[{\widehat{\beta}}]\rho^{-2}$.

\subsubsection{Privacy under Randomized Response}

For given $\varepsilon$, differential privacy requires both
$\PrP\left[d_{i}=1|Y_{i}(1)=1 \right]$ $\leq$ $e^{\varepsilon}\PrP\left[d_{i}=1|Y_{i}(1)=0 \right]$, and $\PrP\left[d_{i}=0|Y_{i}(1)=0 \right]$ $\leq$ $e^{\varepsilon}\PrP\left[d_{i}=0|Y_{i}(1)=1 \right]$. Together, these expressions bound the Bayes factor, which limits how much can learned about the sensitive characteristic upon observation of the collected response.

Making substitutions based on the data-generating model,
\begin{equation}
	1 + \frac{\rho}{(1-\rho)\mu}\leq e^{\varepsilon}
	\label{eq:dp_bayesfactor_1}
\end{equation}
and
\begin{equation}
	1 + \frac{\rho}{(1-\rho)(1-\mu)}\leq e^{\varepsilon}.
	\label{eq:dp_bayesfactor_2}
\end{equation}
For a given choice of $\mu$, the differential privacy guaranteed by randomized response is the maximum of the values of the left-hand sides of equations \eqref{eq:dp_bayesfactor_1} and \eqref{eq:dp_bayesfactor_2}. Hence, privacy loss is minimized when $\mu=\frac{1}{2}$. This is the case we will consider throughout the remaining discussion. We note doing so assumes that inferences about affirmative and negative responses are equally sensitive, which may not always be the case. The results of our analysis do not depend on this assumption. \footnote{These observations highlight another allocation problem: how to trade off protection of affirmative responses for the sensitive item $Y_{i}(1)=1$ against protection of negative responses $Y_{i}(1)=0$.
What do we mean? If $\rho$ is fixed, then increasing $\mu$ reduces the Bayes factor in \eqref{eq:dp_bayesfactor_1} (increasing privacy) and increases the Bayes factor in \eqref{eq:dp_bayesfactor_2} (decreasing privacy). The underlying intuition is fairly simple. Suppose the sensitive question is ``did you lie on your taxes last year?'' Most tax evaders would prefer that their answer not be made public, but non-evaders are probably happy to let the world know they did not cheat on their taxes. In such a setting, with $\rho$ fixed, we can maximize privacy for the tax evader by setting $\mu$ to 1. Recall $\mu$ is the probability of a positive response on the non-sensitive item ($Y_{i}(0)=1$). If $\mu=1$, then when the data report $d_{i}=0, 1$ we know with certainty that $Y_{i}(1)=0$ (i.e., $i$ did not cheat on her taxes). In this special case, the mechanism provides no privacy against inference regarding non-evasion, but maximum attainable privacy (given the mechanism) against inference regarding evasion. This is the role the Bloom filter plays in the full RAPPOR implementation of randomized response \citep{Erlingsson2014}. More generally, the choice of $\mu$ can be tuned to provide relatively more or less privacy against one inference or the other.}

For randomized response, the differential privacy guarantee as a function of $\rho$ is:
\begin{equation}
 	\varepsilon(\rho) = \log\left(1 + \frac{2\rho}{(1-\rho)}\right)=\log\left(\frac{1+\rho}{1-\rho} \right),
 	\label{eq:rand_response_epsilon_func_app}
 \end{equation}
 which follows from setting $\mu=\frac{1}{2}$ in equations \eqref{eq:dp_bayesfactor_1} and \eqref{eq:dp_bayesfactor_2}.

\subsubsection{Statistical Accuracy under Randomized Response}
Expressed as a function of $\rho$, we denote the estimated share of the population with the sensitive characteristic
\begin{equation}
	\widehat{\pi}\left( \rho\right) = \frac{\widehat{\beta}(\rho)-\mu(1-\rho)}{\rho}
\end{equation}
where $\widehat{\beta}(\rho)$ is the population average response when the sensitive question is asked with probability $\rho$. Clearly,
\begin{equation}
	\E[\widehat{\beta}(\rho)] = [\rho\pi + (1-\rho)\mu]
\end{equation}
and
\begin{equation}
	\limfunc{Var}[\widehat{\beta}(\rho)] = \frac{[\rho(\pi-\mu) + \mu](1-\rho(\pi-\mu)-\mu)}{N}.
\end{equation}
It follows that
\begin{equation}
	\limfunc{Var}[\widehat{\pi}(\rho)] = \frac{\limfunc{Var}[\widehat{\beta}(\rho)]}{\rho^{2}} = \frac{[\rho(\pi-\mu) + \mu](1-\rho(\pi-\mu)-\mu)}{\rho^{2}N}.
\end{equation}

% An alternative is to define data quality in terms of relative precision. Here, we have two possibilities. First,
% \begin{align}
% 	RP_{1}(\rho) & = \frac{\limfunc{Var}(\widehat{\pi}\left( 1\right))}{\limfunc{Var}(\widehat{\pi}\left( \rho\right))} \\
% 	         & = \frac{\frac{\pi(1-\pi)}{N}}{\frac{[\rho(\pi-\mu) + \mu](1-\rho(\pi-\mu)-\mu)}{\rho^{2}N}}
% \end{align}
% gives the sampling precision of the population parameter for $\rho$ relative to the sampling precision when $\rho=1$.

% Second, we could define it instead as the sampling precision for the estimated population parameter, $\widehat{\pi}$ relative to the sampling precision of the mean response, holding $\rho$ fixed.
% \begin{align}
%     RP_{2}(\rho) & = \frac{\limfunc{Var}(\widehat{\beta}\left( \rho\right))}{\limfunc{Var}(\widehat{\pi}\left( \rho\right))} \\
%              & = \rho^{2}.
% \end{align}
% This latter relative precision measure tells how much the sampling precision will be overstated if the distortion from randomized response is not taken into account.
We can define data quality as:
\begin{equation}
 	I(\rho) = \limfunc{Var}[\widehat{\pi}\left( 1\right)] - \limfunc{Var}[\widehat{\pi}\left( \rho\right)] .
 	\label{eq:rand_response_dataquality_func}
\end{equation}
This measures the deviation in the sampling variance for the predicted population parameter, $\pi$, relative to the case where there is no privacy protection ($\rho=1$).
% We define data accuracy using this functional form for two reasons. First, it corresponds to expected squared-error loss, which is a standard benchmark in both economics and the computer science literature. Second, this functional form mechanically maps decreases in variance as increases in quality, which is rhetorically useful.

\subsubsection{The Accuracy Cost of Enhanced Privacy under Randomized Response}
%\begin{figure}[th]
%\centerline{\includegraphics[scale=.5]{RandResponse_Plot.pdf}}
%\caption{Production Possibilities under Randomized Response}
%\label{fig:rand_response_ppf}
%\end{figure}

Equations \eqref{eq:rand_response_epsilon_func_app} and \eqref{eq:rand_response_dataquality_func} implicitly define a functional relationship between data privacy, parameterized by $\varepsilon$, and accuracy, parameterized as $I$. This function tells us the marginal cost borne by individuals in the database necessary to achieve an increase in accuracy of the published statistics.
We can characterize the relationship between accuracy, $I$, and privacy loss, $\varepsilon$, analytically. First, we invert equation \eqref{eq:rand_response_epsilon_func_app} to get $\rho$ as a function of $\varepsilon$:
\begin{equation}
 	\rho(\varepsilon) = \frac{e^{\varepsilon}-1}{1+e^{\varepsilon}}.
\end{equation}
Next, we differentiate $I$ with respect to $\varepsilon$ via the chain rule: $\frac{dI}{d\varepsilon} = I^{\prime}(\rho(\varepsilon))\rho^{\prime}(\varepsilon)$:
\begin{equation}
 	I^{\prime}(\rho) = \frac{2\limfunc{Var}[\widehat{\beta}(\rho)]}{\rho} - \frac{(\pi-\frac{1}{2})(1-2\pi)}{N^{2}\rho}.
\end{equation}
and
\begin{equation}
 	\rho^{\prime}(\varepsilon) = \frac{2e^{\varepsilon}}{(1+e^{\varepsilon})^{2}}=\frac{1}{1+cosh(\varepsilon)}.
\end{equation}
Both derivatives are positive, so it follows that $\frac{dI}{d\varepsilon}>0$. A similar derivation shows that $\frac{d^{2}I}{d\varepsilon^{2}}<0$. Increasing published accuracy requires an increase in privacy loss at a rate given by $\frac{dI}{d\varepsilon}>0$. Furthermore, achieving a given increment in accuracy requires increasingly large privacy losses. 

==> optimal.tex <==
% !Tex root = ./abowd-schmutte-privacy_WP.tex
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,sw-edit.tex}
% theory.tex
% Part of abowd-schmutte-privacy.tex



% \subsection{Choosing an Optimal Data Publication Strategy}
% The data custodian could publish, if it wanted to, everything in $D$. Intuitively, this corresponds to the maximum possible -- infinite -- privacy loss. When privacy loss is infinite, there is no error. As we show in Section \ref{sec:}, when there is no privacy loss -- $\varepsilon=0$ error is maximized.

In ``The Pure Theory of Public Expenditure,'' in commenting on the inability of competitive markets to reach an efficient allocation of public goods, \citet{samuelson:1954} observed
\begin{quote}
 The failure of market catallactics in no way denies the following truth: given sufficient knowledge the optimal
decisions can always be found by scanning over all the attainable states of the world and selecting the one which according to the postulated
ethical welfare function is best. The solution "exists"; the problem is how to "find" it.
\end{quote}
The key insight we bring from the formal privacy literature is that the solution to our social choice problem exists. We show there is a well-defined technical relationship between data privacy and accuracy.
We go on to characterize a social welfare function and show, following Samuelson's classic model, how an optimal choice of privacy protection can be made.

% Given access to a differentially private mechanism for publishing data, a statistical agency must choose a privacy guarantee, parameterized by $\varepsilon$. This choice entails an upper bound on the accuracy of the published statistics. Furthermore, there may be an explicit, and well-behaved, production function relating privacy loss and data accuracy. When there is, efficiency dictates that the statistical agency should obtain as much data accuracy as is possible for a given level of privacy loss. However, efficiency does not dictate which level of privacy loss the statistical agency should choose. Our goal is to characterize how the statistical agency should choose the socially optimal level of data privacy.

% Therefore, in this section, we characterize the public good problem faced by the statistical agency following the classic approach of \citet{samuelson:1954}. Data accuracy and privacy
% protection are public goods. The optimal choice will not be obtained through market
% pricing.
%  We therefore ask in this subsection what levels of accuracy and privacy a
% utilitarian social planner would choose to deliver. To obtain this solution, we assume the statistical agency has access to a well-behaved production function with standard properties relating privacy loss and accuracy. 
% We let this section beg the question regarding production possibilities. The main insight from the formal privacy literature is that we can articulate conditions under which this model could feasibly describe the production possibilities faced by the statistical agency. We do so in Section \ref{sec:}.
% As we have already
% discussed, 

\subsection{A General Producer Theory \label{sec:production}}
The statistical agency is in possession of database, $D$, with histogram representation $x$, and must publish answers to query workload, $Q$. 
It also has access to a set of data publication mechanisms. 
Each mechanism entails some bound on privacy loss, $\varepsilon\in[0,\infty]$. 
It also entails a level of data accuracy, $I\in[-\infty,0]$. 
Hence, any mechanism is associated with a pair, $(\varepsilon,I)$. 
Adopting the parlance of producer theory, we refer to each such pair as a \emph{production activity}.
% [This paragraph will raise questions about whether each mechanism is really associated with a single privacy-accuracy pair. We should discuss somewhere, but perhaps not here. ]
Usually in producer theory, a production activity is a vector of inputs and outputs such that the inputs can be transformed into the output. 
Our insight is that the information represented by the database is like an endowment of potential privacy loss. This privacy loss endowment must be expended in some quantity by the data custodian to produce population statistics of a particular accuracy. 

The \emph{transformation set}, $Y=\left\{ \left( \varepsilon ,I \right) \left\vert \varepsilon >0,I<0 \right. \right\}$, describes 
%  a well-defined transformation function between data accuracy, $\alpha$, and
% privacy loss, $\varepsilon$, which we denote $G\left( \varepsilon ,\alpha \right)$.
all feasible production activities. We assume the transformation set has the following properties:
\begin{enumerate}
	\item $Y$ is closed and bounded.
	\item Inactivity is possible, but $\varepsilon>0$ if $I>-\infty$.
\end{enumerate}
Under these assumptions, we can also represent the transformation set in terms of a \emph{transformation function}, $G(\varepsilon,I)$, such that
\begin{equation}
Y=\left\{ \left( \varepsilon ,I \right) \left\vert \varepsilon >0,I<0 \text{ s.t. }G(\varepsilon ,I)\leq0
\right\}\right\}.
\label{eqn:transformation_set}
\end{equation}
The \emph{production frontier} is the set 
\begin{equation}
PF=\left\{ \left( \varepsilon ,I\right)
\left\vert \varepsilon >0,I<0\text{ s.t. }G(\varepsilon ,I)=0\right.
\right\} .  \label{eqn:ppf}
\end{equation}%
Equation (\ref{eqn:ppf}) describes the maximum data accuracy that can be published for a given value of privacy loss. Under our assumptions, it implicitly defines maximum accuracy, $I$, as a function of privacy loss.

\subsubsection*{No Free Lunch}
Scarcity is a key feature of the economic theory of production, often expressed in the axiom of ``no free lunch.'' To produce more of something, you have to give something else up.
As it turns out, there is no free lunch when it comes to data privacy. In separate contributions, \citet{Dwork2004}, \citet{Dwork2008}, and \citet{Kifer:2011:NFL:1989323.1989345} all show that publishing useful data requires an explicit reduction in data privacy. This result holds for any non-trivial definition of formal privacy including, but not restricted to, differential privacy.

\subsection{Preferences \label{sec:preferences}}
We assume a closed system in the sense that data are collected from all members of the population, and all members of the population may benefit directly 
from use of the published statistics. Every person also consumes a set of pure private goods.\footnote{Our analysis assumes the prices of the private goods are exogenous, and we will generally discard them from our notation. Another valid approach would assume data accuracy is an input to production, so that consumer utility depends on accuracy indirectly through its effects on producer prices. We note, finally, that our approach is conceptually distinct from the setting in much of the economics of privacy research, which considers the ability of companies to elicit information about consumers' idiosyncratic preferences and thereby engage in price discrimination. We discuss this related literature in Section \ref{sec:preferences}.} Our formulation allows for arbitrary heterogeneity in preferences for privacy loss and for the accuracy of published statistics. 
 In doing so, we allow for the possibility that one group of people cares primarily about privacy, while getting little or no utility from consuming the data, while another group cares primarily about data accuracy. 

The indirect utility function, $v_{i},$ for each individual is
\begin{equation}
v_{i}\left( y_{i},\varepsilon ,I,p\right) =\max_{q}u_{i}\left(
q,\varepsilon ,I\right) \text{ s.t. }q^{T}p\leq y_{i}
\label{eqn:indirect_utility}
\end{equation}%
where $q$ is the bundle of $L$ private goods chosen by individual $i$ at
prices $p$. The direct utility function $u_{i}\left( q,I,\varepsilon
\right) $, depends upon $q$, the privacy-loss public bad, $\varepsilon $, and
the data-accuracy public good, $I$.

\subsection{The Statistical Agency as a Social Planner}
We assume the statistical agency seeks to maximize a utilitarian social welfare
function%
\begin{equation}
SWF\left( \varepsilon ,I,v,y,p\right) =\sum_{i=1}^{N}v_{i}\left(
y_{i},\varepsilon ,I,p\right)  \label{eqn:swf}
\end{equation}%
where $v$ and $y$ are vectors of $N$ indirect utilities and incomes,
respectively. The agency's problem is to choose $\varepsilon$ and $I$ to solve%
\begin{equation}
\max_{\varepsilon ,I}SWF\left( \varepsilon ,I,v,y,p\right)
\label{eqn:planner}
\end{equation}%
subject to its production set.
Assuming the indirect utility functions are differentiable, the conditions
that characterize the welfare-maximizing levels of $\varepsilon $ and $I$
subject to the feasibility constraint are%
\begin{equation}
\frac{\frac{\partial G\left( \varepsilon ^{0},I^{0}\right) }{\partial
\varepsilon }}{\frac{\partial G\left( \varepsilon ^{0},I^{0}\right) }{%
\partial I}}=\frac{\frac{\partial }{\partial \varepsilon }%
\sum_{i=1}^{N}v_{i}\left( y_{i},\varepsilon ^{0},I^{0},p\right) }{\frac{%
\partial }{\partial I}\sum_{i=1}^{N}v_{i}\left( y_{i},\varepsilon
^{0},I^{0},p\right) }  \label{eqn:optimum}
\end{equation}%
and $G(\varepsilon^{0},I^{0})=0$. The left-hand side of
equation (\ref{eqn:optimum}) is the marginal rate of transformation based on the
production frontier while the right-hand side is the marginal
rate of substitution between privacy loss and data accuracy. We also refer to this as the willingness to accept privacy loss measure in units of published data accuracy.
% See Appendix \ref{app:iu_properties} for the technical details.
A unique solution to the social planner's problem will exist as long as the production set and social welfare function are both convex. 

% \subsubsection{Private Provision is not Optimal}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: abowd-schmutte-privacy
%%% End:

